REGENT: A Retrieval-Augmented Generalist Agent That Can Act In-Context in New Environments

Building generalist agents that can rapidly adapt to new environments is a key challenge for deploying AI in the digital and real worlds. Is scaling current agent architectures the most effective way to build generalist agents? We propose a novel approach to pre-train relatively small policies on relatively small datasets and adapt them to unseen environments via in-context learning, without any finetuning. Our key idea is that retrieval offers a powerful bias for fast adaptation. Indeed, we demonstrate that even a simple retrieval-based 1-nearest neighbor agent offers a surprisingly strong baseline for today's state-of-the-art generalist agents. From this starting point, we construct a semi-parametric agent, REGENT, that trains a transformer-based policy on sequences of queries and retrieved neighbors. REGENT can generalize to unseen robotics and game-playing environments via retrieval augmentation and in-context learning, achieving this with up to 3x fewer parameters and up to an order-of-magnitude fewer pre-training datapoints, significantly outperforming today's state-of-the-art generalist agents. Website: https://kaustubhsridhar.github.io/regent-research

==> tables_jat/just_the_header.tex <==
Env & Num & R\&P & REGENT & REGENT & JAT/Gato & JAT/Gato & JAT/Gato & JAT/Gato & Train \\
 & demos & & & Finetuned & & Finetuned & (All Data) &  (All Data) & From \\
 & & & & & & & &  Finetuned & Scratch \\


==> tables_jat/seen_atari_0.00_all_data.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{c|c|c|c|c}
\hline
Env & Num demos & REGENT & JAT/Gato & JAT/Gato (All Data) \\
\hline
atari-amidar & 5 & 0.96 & 0.02 & 0.06 \\
atari-assault & 5 & 0.02 & 0.02 & 0.08 \\
atari-asterix & 5 & 0.13 & 0.03 & 0.18 \\
atari-asteroids & 5 & 0.07 & 0.0 & 0.0 \\
atari-atlantis & 5 & 0.18 & 0.03 & 0.11 \\
atari-bankheist & 5 & 0.46 & 0.18 & 0.78 \\
atari-battlezone & 5 & 0.47 & 0.01 & 0.05 \\
atari-beamrider & 5 & 0.04 & 0.0 & 0.01 \\
atari-berzerk & 5 & 0.14 & 0.0 & 0.01 \\
atari-bowling & 5 & 1.0 & 1.0 & 1.0 \\
atari-boxing & 5 & 0.22 & 0.38 & 0.96 \\
atari-breakout & 5 & 0.15 & 0.0 & 0.01 \\
atari-centipede & 5 & 0.35 & 0.07 & 0.29 \\
atari-choppercommand & 5 & 0.02 & 0.0 & 0.01 \\
atari-crazyclimber & 5 & 0.19 & 0.14 & 0.59 \\
atari-defender & 5 & 0.1 & 0.01 & 0.08 \\
atari-demonattack & 5 & 0.0 & 0.0 & 0.0 \\
atari-doubledunk & 5 & 0.54 & 0.28 & 0.93 \\
atari-enduro & 5 & 0.0 & 0.0 & 0.05 \\
atari-fishingderby & 5 & 0.62 & 0.1 & 0.58 \\
atari-freeway & 5 & 0.82 & 0.6 & 0.78 \\
atari-frostbite & 5 & 0.44 & 0.01 & 0.28 \\
atari-gopher & 5 & 0.66 & 0.01 & 0.06 \\
atari-gravitar & 5 & 0.03 & 0.06 & 0.21 \\
atari-hero & 5 & 1.0 & 0.17 & 0.27 \\
atari-icehockey & 5 & 0.21 & 0.1 & 0.48 \\
atari-jamesbond & 5 & 0.01 & 0.0 & 0.01 \\
atari-kangaroo & 5 & 0.0 & 0.0 & 0.46 \\
atari-krull & 5 & 0.5 & 0.41 & 0.91 \\
atari-kungfumaster & 5 & 0.0 & 0.02 & 0.0 \\
atari-montezumarevenge & 5 & 0.0 & 0.0 & 0.0 \\
atari-namethisgame & 5 & 0.61 & 0.03 & 0.23 \\
atari-phoenix & 5 & 0.07 & 0.0 & 0.0 \\
atari-pitfall & 5 & 0.97 & 1.01 & 0.98 \\
atari-privateeye & 5 & 0.0 & 0.79 & 0.64 \\
atari-qbert & 5 & 0.57 & 0.01 & 0.13 \\
atari-riverraid & 5 & 0.19 & 0.04 & 0.19 \\
atari-roadrunner & 5 & 0.03 & 0.02 & 0.12 \\
atari-robotank & 5 & 0.23 & 0.04 & 0.13 \\
atari-seaquest & 5 & 0.48 & 0.11 & 0.29 \\
atari-skiing & 5 & 0.0 & 0.0 & 0.03 \\
atari-solaris & 5 & 0.0 & 0.0 & 0.0 \\
atari-surround & 5 & 0.36 & 0.03 & 0.59 \\
atari-tennis & 5 & 0.15 & 0.01 & 0.36 \\
atari-timepilot & 5 & 0.04 & 0.0 & 0.11 \\
atari-tutankham & 5 & 0.16 & 0.02 & 0.57 \\
atari-upndown & 5 & 0.13 & 0.01 & 0.04 \\
atari-venture & 5 & 1.0 & 1.0 & 1.0 \\
atari-videopinball & 5 & 0.0 & 0.01 & 0.03 \\
atari-wizardofwor & 5 & 0.76 & 0.01 & 0.06 \\
atari-yarsrevenge & 5 & 0.01 & 0.01 & 0.03 \\
atari-zaxxon & 5 & 0.14 & 0.01 & 0.09 \\
\hline
Aggregate Mean &  & 0.293 & 0.131 & 0.286 \\
\hline
\end{tabular}
\caption{Values in Figure \ref{fig:seen_atari_0.00_all_data}. Each value is an average across 15 rollouts of different seeds. }
\label{tab:seen_atari_0.00_all_data}
\end{table}

==> tables_jat/seen_babyai_all_data.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{c|c|c|c|c}
\hline
Env & Num demos & REGENT & JAT/Gato & JAT/Gato (All Data) \\
\hline
babyai-action-obj-door & 20 & 0.39 & 0.57 & 0.95 \\
babyai-blocked-unlock-pickup & 20 & 0.45 & 0.97 & 1.0 \\
babyai-boss-level-no-unlock & 20 & 0.49 & 0.1 & 0.49 \\
babyai-boss-level & 20 & 0.49 & 0.1 & 0.49 \\
babyai-find-obj-s5 & 20 & 0.61 & 0.92 & 1.0 \\
babyai-go-to-door & 20 & 0.49 & 0.89 & 0.99 \\
babyai-go-to-imp-unlock & 20 & 0.21 & 0.03 & 0.51 \\
babyai-go-to-local & 20 & 0.66 & 0.46 & 0.94 \\
babyai-go-to-obj-door & 20 & 0.14 & 0.76 & 0.98 \\
babyai-go-to-obj & 20 & 0.14 & 0.76 & 0.98 \\
babyai-go-to-red-ball-grey & 20 & 0.68 & 0.76 & 0.99 \\
babyai-go-to-red-ball-no-dists & 20 & 0.95 & 0.98 & 1.0 \\
babyai-go-to-red-ball & 20 & 0.68 & 0.76 & 0.99 \\
babyai-go-to-red-blue-ball & 20 & 0.71 & 0.71 & 0.95 \\
babyai-go-to-seq & 20 & 0.46 & 0.46 & 0.71 \\
babyai-go-to & 20 & 0.49 & 0.89 & 0.99 \\
babyai-key-corridor & 20 & 0.07 & 0.47 & 0.94 \\
babyai-mini-boss-level & 20 & 0.61 & 0.28 & 0.63 \\
babyai-move-two-across-s8n9 & 20 & 0.0 & 0.0 & 0.02 \\
babyai-one-room-s8 & 20 & 0.96 & 0.97 & 0.99 \\
babyai-open-door & 20 & 0.58 & 0.92 & 1.0 \\
babyai-open-doors-order-n4 & 20 & 0.54 & 0.33 & 0.96 \\
babyai-open-red-door & 20 & 0.99 & 0.99 & 1.0 \\
babyai-open-two-doors & 20 & 0.37 & 0.37 & 1.0 \\
babyai-open & 20 & 0.58 & 0.92 & 1.0 \\
babyai-pickup-above & 20 & 0.44 & 0.86 & 1.01 \\
babyai-pickup-dist & 20 & 0.66 & 0.4 & 1.05 \\
babyai-pickup-loc & 20 & 0.42 & 0.38 & 0.89 \\
babyai-pickup & 20 & 0.44 & 0.86 & 1.01 \\
babyai-put-next-local & 20 & 0.12 & 0.0 & 0.62 \\
babyai-put-next & 20 & 0.12 & 0.0 & 0.62 \\
babyai-synth-loc & 20 & 0.5 & 0.3 & 0.75 \\
babyai-synth-seq & 20 & 0.59 & 0.07 & 0.48 \\
babyai-synth & 20 & 0.5 & 0.3 & 0.75 \\
babyai-unblock-pickup & 20 & 0.25 & 0.23 & 0.85 \\
babyai-unlock-local & 20 & 0.93 & 0.99 & 1.0 \\
babyai-unlock-pickup & 20 & 0.81 & 0.96 & 0.99 \\
babyai-unlock-to-unlock & 20 & 0.35 & 0.79 & 0.85 \\
babyai-unlock & 20 & 0.93 & 0.99 & 1.0 \\
\hline
Aggregate Mean &  & 0.508 & 0.577 & 0.856 \\
\hline
\end{tabular}
\caption{Values in Figure \ref{fig:seen_babyai_all_data}. Each value is an average across 100 rollouts of different seeds. }
\label{tab:seen_babyai_all_data}
\end{table}

==> tables_jat/seen_metaworld_all_data.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{c|c|c|c|c}
\hline
Env & Num demos & REGENT & JAT/Gato & JAT/Gato (All Data) \\
\hline
metaworld-assembly & 100 & 0.83 & 0.89 & 0.98 \\
metaworld-basketball & 100 & 0.68 & 0.03 & 0.02 \\
metaworld-button-press-topdown-wall & 100 & 0.62 & 0.43 & 0.53 \\
metaworld-button-press-topdown & 100 & 0.62 & 0.43 & 0.53 \\
metaworld-button-press-wall & 100 & 0.94 & 0.61 & 0.06 \\
metaworld-button-press & 100 & 0.62 & 0.43 & 0.53 \\
metaworld-coffee-button & 100 & 0.84 & 0.33 & 0.86 \\
metaworld-coffee-pull & 100 & 0.62 & 0.01 & 0.15 \\
metaworld-coffee-push & 100 & 0.18 & 0.04 & 0.46 \\
metaworld-dial-turn & 100 & 0.83 & 0.33 & 0.94 \\
metaworld-disassemble & 100 & 2.24 & 0.0 & 0.15 \\
metaworld-door-close & 100 & 1.0 & 0.46 & 0.97 \\
metaworld-door-open & 100 & 0.98 & 0.46 & 0.89 \\
metaworld-drawer-close & 100 & 1.0 & 0.89 & 0.95 \\
metaworld-drawer-open & 100 & 0.96 & 0.91 & 0.98 \\
metaworld-faucet-close & 100 & 0.53 & 0.16 & 0.94 \\
metaworld-faucet-open & 100 & 0.99 & 0.68 & 0.94 \\
metaworld-hammer & 100 & 0.95 & 0.52 & 0.98 \\
metaworld-handle-press-side & 100 & 0.99 & 0.83 & 0.83 \\
metaworld-handle-press & 100 & 0.99 & 0.83 & 0.83 \\
metaworld-handle-pull-side & 100 & 0.48 & 0.0 & 0.6 \\
metaworld-handle-pull & 100 & 0.48 & 0.0 & 0.6 \\
metaworld-lever-pull & 100 & 0.19 & 0.03 & 0.07 \\
metaworld-peg-insert-side & 100 & 0.7 & 0.15 & 0.85 \\
metaworld-peg-unplug-side & 100 & 0.31 & 0.02 & 0.06 \\
metaworld-pick-out-of-hole & 100 & 0.01 & 0.0 & 0.0 \\
metaworld-pick-place-wall & 100 & 0.99 & 0.01 & 0.08 \\
metaworld-pick-place & 100 & 0.99 & 0.01 & 0.08 \\
metaworld-plate-slide-back-side & 100 & 1.0 & 0.02 & 0.97 \\
metaworld-plate-slide-back & 100 & 1.0 & 0.02 & 0.97 \\
metaworld-plate-slide-side & 100 & 0.99 & 0.19 & 0.13 \\
metaworld-plate-slide & 100 & 1.0 & 0.02 & 0.97 \\
metaworld-push-back & 100 & 0.84 & 0.01 & 0.96 \\
metaworld-push-wall & 100 & 0.81 & 0.01 & 0.21 \\
metaworld-push & 100 & 0.84 & 0.01 & 0.96 \\
metaworld-reach-wall & 100 & 0.99 & 1.03 & 0.93 \\
metaworld-reach & 100 & 0.99 & 1.03 & 0.93 \\
metaworld-shelf-place & 100 & 0.96 & 0.0 & 0.81 \\
metaworld-soccer & 100 & 0.61 & 0.21 & 0.8 \\
metaworld-stick-pull & 100 & 0.88 & 0.04 & 0.78 \\
metaworld-stick-push & 100 & 0.75 & 0.02 & 0.18 \\
metaworld-sweep-into & 100 & 0.91 & 0.16 & 0.99 \\
metaworld-sweep & 100 & 0.91 & 0.16 & 0.99 \\
metaworld-window-close & 100 & 0.9 & 0.1 & 0.94 \\
metaworld-window-open & 100 & 0.97 & 0.14 & 1.0 \\
\hline
Aggregate Mean &  & 0.82 & 0.281 & 0.653 \\
\hline
\end{tabular}
\caption{Values in Figure \ref{fig:seen_metaworld_all_data}. Each value is an average across 100 rollouts of different seeds. }
\label{tab:seen_metaworld_all_data}
\end{table}

==> tables_jat/seen_mujoco_all_data.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{c|c|c|c|c}
\hline
Env & Num demos & REGENT & JAT/Gato & JAT/Gato (All Data) \\
\hline
mujoco-ant & 100 & 0.17 & 0.12 & 0.98 \\
mujoco-doublependulum & 100 & 0.02 & 0.01 & 0.59 \\
mujoco-humanoid & 100 & 0.02 & 0.02 & 0.08 \\
mujoco-pendulum & 100 & 0.06 & 0.03 & 0.42 \\
mujoco-pusher & 100 & 0.9 & 0.95 & 1.01 \\
mujoco-reacher & 100 & 0.9 & 0.91 & 0.97 \\
mujoco-standup & 100 & 0.26 & 0.2 & 0.42 \\
mujoco-swimmer & 100 & 0.82 & 0.97 & 1.04 \\
mujoco-walker & 100 & 0.05 & 0.16 & 0.75 \\
\hline
Aggregate Mean &  & 0.356 & 0.374 & 0.696 \\
\hline
\end{tabular}
\caption{Values in Figure \ref{fig:seen_mujoco_all_data}. Each value is an average across 100 rollouts of different seeds. }
\label{tab:seen_mujoco_all_data}
\end{table}

==> tables_procgen/just_the_3_headers_procgen.tex <==
% table_id_p_0.1_checkpoints.tex
Env & sticky prob & num demos & (epoch, end batch) & \Regent{} & \rnp{}\\

% table_id_p_0.1_figure_values.tex
Env & sticky prob & num demos & (epoch, end batch) & \Regent{} & \rnp{} & \Regent{} (seen levels)\\

% table_ood_p_0.2_figure_values.tex
Env & sticky prob & num demos & (epoch, end batch) & \Regent{} & \rnp{} & MTT \citep{mtt}\\


==> tables_procgen/table_id_p_0.1_checkpoints.tex <==
\begin{table}[H]
\centering
\scriptsize
\begin{tabular}{llllll}
\toprule
 &  &  &  & Regent & RandP \\
\midrule
\multirow[t]{3}{*}{bigfish} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (25.7, None) & (14.98, None) \\
 &  &  & (1, 11612) & (28.46, None) &  \\
 &  &  & (2, 11612) & (23.62, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{bossfight} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (5.6, None) & (2.1, None) \\
 &  &  & (1, 11612) & (3.44, None) &  \\
 &  &  & (2, 11612) & (2.56, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{caveflyer} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (7.68, None) & (3.37, None) \\
 &  &  & (1, 11612) & (8.22, None) &  \\
 &  &  & (2, 11612) & (7.94, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{chaser} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (2.4, None) & (1.72, None) \\
 &  &  & (1, 11612) & (2.45, None) &  \\
 &  &  & (2, 11612) & (2.59, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{coinrun} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (8.2, None) & (6.9, None) \\
 &  &  & (1, 11612) & (7.8, None) &  \\
 &  &  & (2, 11612) & (7.6, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{dodgeball} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (7.12, None) & (4.03, None) \\
 &  &  & (1, 11612) & (6.4, None) &  \\
 &  &  & (2, 11612) & (7.16, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{fruitbot} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (16.36, None) & (7.05, None) \\
 &  &  & (1, 11612) & (17.0, None) &  \\
 &  &  & (2, 11612) & (16.08, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{heist} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (7.2, None) & (7.3, None) \\
 &  &  & (1, 11612) & (5.6, None) &  \\
 &  &  & (2, 11612) & (7.0, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{leaper} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (9.2, None) & (7.17, None) \\
 &  &  & (1, 11612) & (8.2, None) &  \\
 &  &  & (2, 11612) & (9.0, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{maze} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (8.4, None) & (6.6, None) \\
 &  &  & (1, 11612) & (6.0, None) &  \\
 &  &  & (2, 11612) & (5.8, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{miner} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (6.58, None) & (3.84, None) \\
 &  &  & (1, 11612) & (5.82, None) &  \\
 &  &  & (2, 11612) & (4.86, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\multirow[t]{3}{*}{starpilot} & \multirow[t]{3}{*}{p=0.1} & \multirow[t]{3}{*}{n=20} & (0, 11612) & (16.1, None) & (12.32, None) \\
 &  &  & (1, 11612) & (12.38, None) &  \\
 &  &  & (2, 11612) & (12.98, None) &  \\
\cline{1-6} \cline{2-6} \cline{3-6}
\bottomrule
\end{tabular}
\caption{Returns in seen levels in seen envs for various checkpoints. Each value is an average across 10 levels with 5 rollouts each with $p_{\text{sticky}}=0.1$)}
\label{tab:id_p_0.1_checkpoints}
\end{table}
